MultiOrg: A Multi-rater Organoid-detection Dataset

High-throughput image analysis in the biomedical domain has gained significant attention in recent years, driving advancements in drug discovery, disease prediction, and personalized medicine. Organoids, specifically, are an active area of research, providing excellent models for human organs and their functions. Automating the quantification of organoids in microscopy images would provide an effective solution to overcome substantial manual quantification bottlenecks, particularly in high-throughput image analysis. However, there is a notable lack of open biomedical datasets, in contrast to other domains, such as autonomous driving, and, notably, only few of them have attempted to quantify annotation uncertainty. In this work, we present MultiOrg a comprehensive organoid dataset tailored for object detection tasks with uncertainty quantification. This dataset comprises over 400 high-resolution 2d microscopy images and curated annotations of more than 60,000 organoids. Most importantly, it includes three label sets for the test data, independently annotated by two experts at distinct time points. We additionally provide a benchmark for organoid detection, and make the best model available through an easily installable, interactive plugin for the popular image visualization tool Napari, to perform organoid quantification.

==> body/03_dataset/fig_inter_rater_at_t1.tex <==
\begin{figure}[ht]
    \centering
\includegraphics[width=1.0\columnwidth]{body/03_dataset/fig/inter_rater_t1_A_vs_t1_B.png}
    \caption{Inter-rater F1-score (left), Precision (middle), and Recall (right) on the test set between $test^1_A$ and $test^1_B$, where $test^1_A$ is considered the \eac{GT},  split according to study type.
    Raters agree more on 'Normal' images, indicating that the annotation of 'Macros' images is more challenging.
    Inter-rater scores are generally lower than inter-rater scores (\Cref{fig:intra_rater})}
    \label{fig:inter-rater-t1}
\end{figure}


% Another observation in line with the above can be drawn by studying \Cref{tab:multi-rater-analysis} , where higher F1-scores are found between annotations from time point $^1$ (mean on the two subsets is 0.610 and 0.710 for $test^1_A$ vs. $test^1_B$, compared to 0.586 and 0.561 for $test^0$ vs. the subsets at timepoint $t^1$). Naturally, intra-rater scores are higher than inter-rater scores (annotators agree more with themselves at a new timepoint that with others

==> body/03_dataset/fig_intra_inter_rater_old.tex <==
\begin{figure}[ht]
    \centering
\includegraphics[width=1.0\columnwidth]{body/03_dataset/fig/intra-and-inter-rater.png}
    \caption{ 
    F1 Score(left), Precision(middle), and Recall(right) shown for Intra- and Inter-rater scores for both annotators. Scores are split for the two test subsets and according to experimental type. For computing these scores $test^0$ is always considrered the \eac{GT}. The intra-rater scores indicate that Annotator A is more consistent in time, especially for the Normal experiments (higher intra-rater scores). Both intra- and inter-rater plots show an overall higher precision and lower recall, indicating that $test^0$ has many more annotations which are treated here as \eac{FNs}, confirming the statistics of \cref{tab:train-test-numbers} that at time point $t^1$ both annotators reduced the number of annotatos. This may indicate annotation improvement over time, since qualitative observations of the label set $test^0$ also suggested that the pseudo labels used as a starting point for all annotations were not manually removed. Another observation in line with the above can be drawn by studying \Cref{tab:multi-rater-analysis} , where higher F1-scores are found between annotations from time point $^1$ (mean on the two subsets is 0.610 and 0.710 for $test^1_A$ vs. $test^1_B$, compared to 0.586 and 0.561 for $test^0$ vs. the subsets at timepoint $t^1$). Naturally, intra-rater scores are higher than inter-rater scores (annotators agree more with themselves at a new timepoint that with others).}
    \label{fig:intra-inter_rater}
\end{figure}

==> body/03_dataset/fig_intra_rater.tex <==
\begin{figure}[ht]
    \centering
\includegraphics[width=1.0\columnwidth]{body/03_dataset/fig/intra_rater.png}
    \caption{ 
    Intra-rater F1-score (left), Precision (middle), and Recall (right), where $test^0$ is considered the \eac{GT}, for both annotators and according to study type.
    Annotator A appears more consistent when reannotating 'Normal' images (higher scores).
    Annotation of 'Macros' is more challenging (lower score).
    Both annotators show an overall higher Precision and Lower recall, indicating that $test^0$ has many more annotations which are treated here as \eac{FNs}.
% (the spurious $t^0$ annotations become here \eac{FNs})
    }
    \label{fig:intra_rater}
\end{figure}



 % The intra-rater scores indicate that Annotator A is more consistent in time, especially for the Normal experiments (higher intra-rater scores). Both intra- and inter-rater plots show an overall higher precision and lower recall, indicating that $test^0$ has many more annotations which are treated here as \eac{FNs}, confirming the statistics of \cref{tab:train-test-numbers} that at time point $t^1$ both annotators reduced the number of annotatos. This may indicate annotation improvement over time, since qualitative observations of the label set $test^0$ also suggested that the pseudo labels used as a starting point for all annotations were not manually removed. Another observation in line with the above can be drawn by studying \Cref{tab:multi-rater-analysis} , where higher F1-scores are found between annotations from time point $^1$ (mean on the two subsets is 0.610 and 0.710 for $test^1_A$ vs. $test^1_B$, compared to 0.586 and 0.561 for $test^0$ vs. the subsets at timepoint $t^1$). Naturally, intra-rater scores are higher than inter-rater scores (annotators agree more with themselves at a new timepoint that with others)

==> body/03_dataset/tab_test_overview.tex <==
\begin{table}[ht]
    \caption{An overview of the images of the test set and organoid numbers in the three label sets, split according to annotator (A and B) and experiment type (Normal and Macros)}
    \label{tab:testest-numbers}
    \centering
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{| *{10}{c|} }
            \hline
                                    Experimental Setup
                                   & \multicolumn{2}{c|}{Normal}
                                   & \multicolumn{2}{c|}{Macros} 
                                   & \multicolumn{2}{c|}{Combined}
                                   \\
            \hline
            %\textbf{t0\_AB} & Images                        & Organoids     & Images      & Organoids    & Images      & Organoids      \\
             Test set & Images & Organoids     & Images      & Organoids    & Images      & Organoids      \\
            \hline
            $test^{0}_{A}$   & 8   & 1145            & 14         & 1865        & 22          & 3010                         \\
            \hline
            $test^{0}_{B}$   & 20    & 3020           & 13        & 1493         & 33          &   4513                      \\
            \hline
            \textbf{$test^{0}$}  & 28 & 4165    & 27 & 3358 & 55 & 7523        \\
            \hline
            \hline
            %\textbf{t1\_A} & Images                        & Organoids     & Images      & Organoids      & Images      & Organoids      \\
            %\hline
            
            \textbf{$test^{1}_{A}$}         & 28       & 2748           & 27     & 1981      & 55   & 4729                  \\
            \hline
            

            %\textbf{t1\_B} & Images                        & Organoids      & Images      & Organoids     & Images      & Organoids     \\
            %\hline
            \textbf{$test^{1}_{B}$}       & 28          & 2655         & 27          & 2301      & 55   & 4956                     \\
            \hline
        \end{tabular}
    }
\end{table}

    % \textbf{i)} The average organoid size in t0\_AB for Normal, Macros and combined images annotated by Annotator A are \SI{11,887}{\micro\meter\squared}, \SI{4,891 }{\micro\meter\squared}, and \SI{7,552}{\micro\meter\squared} respectively.For Annotator B, it is \SI{17,064}{\micro\meter\squared}, \SI{9,654}{\micro\meter\squared} and \SI{14,613}{\micro\meter\squared} respectively.\textbf{ii)} The average organoid size in t1\_A for Normal, Macros and combined images are \SI{19,413}{\micro\meter\squared}, \SI{8,714}{\micro\meter\squared}, and \SI{14,931}{\micro\meter\squared} respectively. textbf{iii)} The average organoid size in t1\_B for Normal, Macros and combined images are\SI{21,316}{\micro\meter\squared}, \SI{8,187}{\micro\meter\squared}, and \SI{15,220}{\micro\meter\squared} respectively.

==> body/04_baseline/042_inference.tex <==
\subsection{Inference procedure}


==> body/04_baseline/044_model_availability.tex <==
\subsection{Model availability}
probably it should be available both in napari and as a Python pkg

==> flow/latex_evangelium.tex <==
\section{Latex evangelium}
\label{sec:evangelium}
% \label{sec:formatting}

Look at the .tex file to fully understand this \Cref{sec:evangelium}!


\subsection*{labels and referencing}
\begin{itemize}
    \item label sections that are supposed to be referenced with \label{sec:section_name}
    \item label figures with \label{fig:figure_name}
    \item label tables with \label{tab:table_name}
    \item label equations with \label{eq:equation_name}
    \item reference with \cref{sec:evangelium} or \Cref{sec:evangelium}
\end{itemize}

\subsection*{figures, tables and equations}
\begin{itemize}
    \item use a separate .tex file for each figure/table; this will make the final layout/typesetting process much smoother as we can easily move them around
    \item we put figures in a subfolder for each section called /fig
    \item observe the above label instructions
\end{itemize}

\subsection*{citations}
\begin{itemize}
    \item for citations we use \citep{kofler2023approaching} or \citet{kofler2023approaching}
\end{itemize}

\subsection*{acronyms}
\begin{itemize}
    \item we define acronyms in /flow/acronyms.tex
    \item for singular acronyms use \eac{CNN} or \eacf{CNN}.
    \item for plural acronyms we use \eacp{CNN} or \eacfp{CNN}.
\end{itemize}

\subsection*{misc but important}
\begin{itemize}
    \item we write in the present tense
    \item we actively use spellcheckers such as Grammarly
    \item we use auto code formatting and lining
    \item we use one line of code for each sentence to enable proper version control with git
\end{itemize}


==> head/keywords.tex <==
\keywords{
    machine learning,
    deep learning,
    model selection,
    training set,
    validation set,
    overfitting,
    [TODO]
}

